Quantized Zero Dynamics Attacks against Sampled-data Control Systems

For networked control systems, cyber-security issues have gained much attention in recent years. In this paper, we consider the so-called zero dynamics attacks, which form an important class of false data injection attacks, with a special focus on the effects of quantization in a sampled-data control setting. When the attack signals must be quantized, some error will be necessarily introduced, potentially increasing the chance of detection through the output of the system. In this paper, we show however that the attacker may reduce such errors by avoiding to directly quantize the attack signal. We look at two approaches for generating quantized attacks which can keep the error in the output smaller than a specified level by using the knowledge of the system dynamics. The methods are based on a dynamic quantization technique and a modified version of zero dynamics attacks. Numerical examples are provided to verify the effectiveness of the proposed methods.

==> workspace/abstract.tex <==
For networked control systems, cyber-security issues have gained much attention in recent years. In this paper, we consider the so-called zero dynamics attacks, which is a form of false data injection attacks, with a special focus on the effects of quantization in the sampled-data control setting. When the attack signals must be quantized, some error will be necessarily introduced, potentially increasing the chance of detection through the output of the system. In this paper, we show however that the attacker may reduce such errors by avoiding to directly quantize the attack signal. We look at two approaches for generating quantized attacks which can keep the error in the output smaller than a specified level by using the knowledge of the system dynamics. The methods are based on a dynamic quantization technique 
and a modified version of zero dynamics attacks. Numerical examples are provided to verify the effectiveness of the proposed methods.

==> workspace/conclusion.tex <==
\section{Conclusion}\label{ch:conclusion}
%In this paper, we proposed the attack method to deviate a system state while reducing an output error, where an input of a sampled-data system is quantized. At that time, we considered a system which has unstable zeros.\par
%We proposed two types of method. The first method modifies the conventional zero dynamics attack by the dynamic quantizer. The second method directly calculates the quantized attack. These methods achieve the goal to deviate a system state. However, the effect on a system output is not same. Though the former method is less influential when the zero dynamics attack is statically quantized, the effect on an output depends on the number of unstable zeros in a system and its values. On the other hand, the latter method is independent of them. Moreover, its effect on an output is less than the former method.\par
%Future work is to propose the quantized attack method on a feedback condrol system. In this paper, we assumed a feedforward control system. So we were able to consider the effect of the quantized attack independently of control law. On the other hand, in a feedback control system, the quantization of the attack affects not only the system output but also the control input, so the problem formulation become more complicated. However, since a feedback control system is widely used in practical applications, this seems to be an important issue.

In this paper, we have studied the effects of quantization on sampled-data systems under zero dynamics attacks. We have proposed methods for generating quantized attacks exploiting the unstable zeros in the plant after discretization. Under these attacks, the system state diverges while the error in the output due to quantization is kept small. 
In particular, we have proposed two types of methods. The first one utilizes the conventional zero dynamics attacks and modifies such attack signals by dynamic quantization. In contrast, in the second method, slightly modified version of zero dynamics attacks is 
quantized. These methods have been compared with the simple
approach of directly quantizing the conventional zero
dynamics attacks, and our analysis shows the they perform
strictly better. 

Our study in this paper has been limited in two respects.
One is that the system is assumed to have unstable zeros.
The case without such zeros can be handled if there are
redundancy in the inputs compared to the outputs 
\cite{zsa}, and we will pursue such an approach.
The other is that the control system setting is in the 
feedforward form. 
Hence, for our future work, we must look at the feedback control case, where the chosen control laws may affect the performance of the quantized attack. We should note that these two system settings have been separately treated for the dynamic quantization in the literature \cite{dquant}. This may indicate the differences in the nature of the problems.


==> workspace/dq.tex <==
\section{Dynamic quantization}\label{ch:dq}
In this section, we briefly introduce the method called dynamic quantization from the works \cite{dquant,dqseri,sythdq}. 

We consider the two feedforward discrete-time systems shown in Figs.~\ref{fig:dq:osys} and \ref{fig:dq:qsys}, 
where the controllers apply the same input $u[k]$ 
to both systems. The plant is from \eqref{eq:pr:dsys} 
without the attack signal, i.e., $b[k]\equiv0$. 
The difference between the two systems is that the 
first system in Fig.~\ref{fig:dq:osys} is the original 
one with the ideal output denoted by $y_I$ whereas 
in the second system in Fig.~\ref{fig:dq:qsys}, 
the input is quantized, resulting in the output 
$y$ with some errors from $y_I$. 
The problem is to find a quantizer with dynamics 
to minimize the error $y-y_I$ based on the past 
inputs $u[k]$ and their quantized values $v[k]$.
In particular, the measure of output error is defined as
\begin{equation}
    E(Q) = \sup_{u,k}\left|y[k]-y_I[k]\right|.
\label{eq:dq:error}
\end{equation}\par


\begin{figure}[t]
    \begin{minipage}[t]{1\linewidth}
\vspace*{1mm}
        \centering        
\includegraphics[width=0.7\linewidth]{workspace/picture/dq_osys.png}
\vspace*{1mm}
        \caption{Controller and plant}
        \label{fig:dq:osys}
    \end{minipage}
    \vspace{0.04\linewidth}
    \\
    \begin{minipage}[t]{1\linewidth}
        \centering
     \includegraphics[width=1\linewidth]{workspace/picture/dq_qsys.png}
\vspace*{1mm}
        \caption{Controller and plant with an input quantizer}
        \label{fig:dq:qsys}
    \end{minipage}
\end{figure}

Before we proceed to dynamic quantizers, we can
look at the case of static quantization 
when the input $u[k]$ 
is directly quantized as $v[k]=q(u[k])$.
%i.e., with $G=O$ and $H=I$ in \eqref{eq:dq:dquant}, 
In this case, it is known that 
the output error \eqref{eq:dq:error} can be obtained as 
\begin{equation}
 E(Q)
  = \frac{1}{2}\sum\limits_{k=0}^\infty\left|CA^kB\right| d.
\label{eq:dq:staticeps}
\end{equation}
Since the plant is assumed to be stable, this value is
finite. This formula suggests that for systems with
slower convergence, quantization has larger impact
on the output, and moreover this error is linear with
respect to the quantization width $d$.




\subsection{Basic structure of dynamic quantizers}\label{se:dq}
Here, we assume that the plant is minimum phase, i.e., its zeros are stable.\par
The dynamic quantizer is given by a linear system whose output is quantized by the uniform quantizer in Section \ref{se:plant}:
\begin{equation}
    Q\left\{
    \begin{aligned}
    \xi[k+1]&=E\xi[k]+F_1v[k]+F_2u[k],\\
    v[k]&=q(G\xi[k]+Hu[k]),
    \end{aligned}
    \right.\label{eq:dq:dquant}
\end{equation}
where the initial state is given by $\xi[0]=0$. 
We would like to design the dynamic quantizer 
so as to minimize the output error in \eqref{eq:dq:error}.

The dynamic quantizer is known to be optimal if
\begin{equation}
  \begin{split}
     E&=A,~~F_1=-F_2=B,\\
     G&=-\frac{CA}{CB},~~H=I
    \end{split}
\label{eq:dq:param}
\end{equation}
and then the minimum output error is given by \cite{dquant}
\begin{equation}
    E(Q)=\frac{1}{2}\left|CB\right|d.
\label{eq:dq:erroropt}
\end{equation}
It is obvious that with dynamic quantization,
the output error becomes strictly smaller than
that for the static case in \eqref{eq:dq:staticeps}.
In particular, $E(Q)$ in \eqref{eq:dq:erroropt} is
independent of the system matrix $A$. So different from
the static case, the output error does not depend on
the convergence rate of the plant.

However, we must note that this design method can be 
applied only to minimum phase systems. 
In fact, when the system \eqref{eq:pr:dsys} has 
unstable zeros, the dynamic quantizer outlined 
above becomes unstable. The case for nonminimum 
phase systems is discussed next. 

\subsection{Dynamic quantizer based on serial decomposition}\label{se:dqseri}
We describe the dynamic quantization approach of 
\cite{dqseri} based on decomposition of the plant. 
Suppose that the system \eqref{eq:pr:dsys} has unstable zeros. We denote by $P$ the system from the quantized input $v[k]$ to the output $y[k]$ in \eqref{eq:pr:dsys}. This is decomposed serially to subsystems $P_s$ and $P_u$ as $P=P_s\cdot P_u$ such that the following hold:
\begin{enumerate}
    \item $P_s$ is stable, minimum phase and strictly proper, and
    \item $C_sB_s\neq0$,
\end{enumerate}
where the realizations of $P_s$ and $P_u$ are, respectively, given by $(A_s,B_s,C_s,0)$ and $(A_u,B_u,C_u,D_u)$. Note that the minimum phase property of $P_s$ implies that $A_s-\frac{B_sC_sA_s}{C_sB_s}$ is a stable matrix\cite{dquantstable}.\par
Dynamic quantization based on serial decomposition generates the quantized signal $v[k]$ as follows:
\begin{equation}
  Q_s\left\{
    \begin{aligned}
    \xi[k+1]
      &= A_s\xi[k]+B_sv[k]-B_su[k], \\
    v[k]
      &= q\left(-\frac{C_sA_s}{C_sB_s}\xi[k]+u[k]\right).
    \end{aligned}
  \right.
\label{eq:dq:dqseri}
\end{equation}
Notice that this is the optimal quantizer for the system $P_s$
for \eqref{eq:dq:param}.
The output error in \eqref{eq:dq:error} for this case 
can be expressed as
\begin{equation}
E(Q_s)
 = \frac{1}{2}\left\|P_u\right\|_{i_\infty}
    \left|C_sB_s\right|d,
\label{eq:dq:dqserierroropt}
\end{equation}
where $\left\|P_u\right\|_{i\infty}$ is the induced-$l_\infty$ norm of the subsystem $P_u$ given by
\begin{equation}
    \left\|P_u\right\|_{i\infty}:=\sup\limits_{r\in l_\infty,r\neq0}\frac{\left\|P_ur\right\|_\infty}{\left\|r\right\|_\infty}.\label{eq:dq:linfnorm}
\end{equation}
This is the contribution of $P_u$ to the output error 
in \eqref{eq:dq:dqserierroropt}.

Note that in this method, there is some freedom in the choices of the subsystems $P_s$ and $P_u$. One difficulty is that if $P$ has multiple unstable zeros, then the optimal way of decomposition is not known in general. One exception is when the plant $P$ has only one unstable zero. In that case, the optimal decomposition and output error can be obtained explicitly. Let $\lambda$ be the unstable zero $(|\lambda|>1)$ of $P$. Then, $P_u$ should be taken in transfer function form as $P_u(z)=(z-\lambda)/z$. The optimal output error can be obtained as
\begin{equation}
    E(Q_s)=\frac{1}{2}(1+\left|\lambda\right|)\left|C_sB_s\right|d.\label{eq:dq:dqseriopt}
\end{equation}




==> workspace/inputred.tex <==
\section{Quantized attack for an input redundant system}\label{ch:inputred}
In this section, we explain the quantized attack $\{b[k]\}_{k=0}^{\infty}$ where the system \eqref{eq:csys} satisfies following condition.
\begin{itemize}
    \item $N>1$
\end{itemize}
Concretely, we propose the two types of methods.
\begin{enumerate}
    \item the method modifies the continuous attack by using the dynamic quantizer to reduce influence on the output
    \item the method directly search the attack which satisfies the conditions at each time.
\end{enumerate}
The attack by first method reduces the output error compared with the case where the attack is statically quantized. Moreover, if $A-B(CB)^{-1}CA$ is a stable matrix, then we obtain the optimal the dynamic quantizer unlike the method in \ref{se:dqzda}. The attack by second method solves a lattice searching problem at each sampling time. That means this method requires high computational costs. However, this method probably achieve less output error compared with the first method. Therefore, there is the trade-off of the first and second method. Though the lower limit of the output error by the second method is not revealed, there exists the numerical example where the second method achieves better performance than the first method.\par
If $N>1$, the system \eqref{eq:csys} can be equivalently expressed as the lifted system given by
\begin{equation}
\begin{split}
    \tilde{x}[k+1]&=\tilde{A}\tilde{x}[k]+\tilde{B}_N(v[k]+b[k]),\\
    y[k]&=\tilde{C}\tilde{x}[k],
\end{split}\label{eq:re:syslift}
\end{equation}
where $\tilde{x}[k]:=x[Nk]=x(NkT)$. The lifted form of the control input $v[k]$ is 
\begin{equation}
    \tilde{v}[k]:=\begin{bmatrix}   
    v[Nk] \\
    \vdots \\
    v[N(k+1)-1]
    \end{bmatrix}.\label{eq:re:vlift}
\end{equation}
Analogously, other signals $u[k]$, $b[k]$, $a[k]$ can be transformed. Define $\tilde{A}:=A^N$, $\tilde{B}_l:=[A^{l-1}B\cdots B]$, $\tilde{C}:=C$ by using the system matrices $A$ and $B$ in \eqref{eq:pr:dsys}.\par
If the input is not quantized and either $\tilde{A}-\tilde{B}_N(\tilde{C}\tilde{B}_N)^+\tilde{C}\tilde{A}$ or $A-B(CB)^{-1}CA$ is unstable, then zero dynamics attack in \ref{se:zda} or the attack by \eqref{eq:no:zdag} in \ref{se:calc} is $\epsilon$-stealthy and $\{H_k\}_{k=0}^{\infty}$-disruptive with respect to the given scalar $\epsilon>0$ and the sequence $\{H_k\}_{k=0}^{\infty}$. Here, $(\tilde{C}\tilde{B}_N)^+$ is the pseudo inverse of $\tilde{C}\tilde{B}_N$. Note that zero dynamics attack is implemented as follows when $\tilde{A}-\tilde{B}_N(\tilde{C}\tilde{B}_N)^+\tilde{C}\tilde{A}$ is unstable. First, calculate the attack $\{\tilde{a}[k]\}_{k=0}^{\infty}$ with respect to the lifted system \eqref{eq:re:syslift}. At that time, $\tilde{a}[k]\in\mathbb{R}^{Nm}$ for every $k$. After that, the attack $\{a[k]\}_{k=0}^{\infty}$ is given by
\begin{equation*}
    \begin{bmatrix}
        a[Nk]\\
        \vdots \\
        a[Nk+N-1]
    \end{bmatrix}=\tilde{a}[k].
\end{equation*}
Above manipulation is the inverse of lifting.\par
However, if the above matrices are stable, zero dynamics attack and the attack by \eqref{eq:no:zdag} may not be $\{H_k\}_{k=0}^{\infty}$-disruptive. Therefore, the attack method which achieve $\epsilon$-stealthiness with respect to $\epsilon=0$ and $\{H_k\}_{k=0}^{\infty}$-disruption is proposed by taking advantage of the input redundancy, which is called zero stealthy attack (ZSA) \cite{zsa}.

\subsection{Zero stealthy attack}\label{se:zsa}
Consider the situation where the input is not quantized, which means $\tilde{v}[k]=\tilde{u}[k]$, $\tilde{b}[k]=\tilde{a}[k]$. At first, deal with the difference between the output under the attack and the attack-free output. Denote $\Delta\tilde{x}[k]:=\tilde{x}_{u+a}[k]-\tilde{x}_u[k]$, $\Delta \tilde{y}[k]:=\tilde{C}\Delta\tilde{x}[k]$, then
\begin{equation}
    \begin{split}
    \Delta\tilde{x}[k+1]&=\tilde{A}\Delta\tilde{x}[k]+\tilde{B}_N\tilde{a}[k],\\
    \Delta\tilde{y}[k]&=\tilde{C}\Delta\tilde{x}[k],
    \end{split}\notag%\label{eq:re:difflift}
\end{equation}
where $\Delta\tilde{x}[0]=0$. Define the attack $\{a[k]\}_{k=0}^{\infty}$ as following form.
\begin{equation}
     \tilde{a}[k]=\kappa_k\eta+\xi_k\label{eq:re:atk}
\end{equation}
Here, $\kappa_k\in\mathbb{R}$, $\eta$, $\xi_k\in\mathbb{R}^{mN}$.\par
Consider the difference between the outputs $\Delta\tilde{y}[k]$. If the parameters are defined as follows, then the attack is $\epsilon$-stealthy with respect to $\epsilon=0$.
\begin{equation}
    \begin{split}
    &\tilde{C}\tilde{B}_N \eta=0\\
    &\tilde{C}\tilde{B}_N\xi_k+\tilde{C}\tilde{A}\Delta\tilde{x}[k]=0
    \end{split}\notag
\end{equation}\par
Let us move on to the difference between the states $\Delta\tilde{x}[k]$. In the sequel, the sequence $\{h_k\}_{k=0}^{\infty}$ is given. Moreover, the time sequence $\{t_k\}_{k=0}^{\infty}$ is of the form; $t_k=TN(k+\theta_k)$. We consider the condition for the attack $\{b[k]\}_{k=0}^{\infty}$ such that $\left\|x_{u+a}(t_k)-x_u(t_k)\right\|>=h_k$. For every $t_k$, the difference between the states is denoted $x_{u+a}(t_k)-x_u(t_k)=\bar{A}\Delta\tilde{x}[k]+\Phi_k\tilde{a}[k]$ by using following matrices.
\begin{equation}
    \begin{split}   
    \bar{A}_k&:=e^{A_c\theta_kNT}\\
    \Phi_k&:=[\Phi_k(1),\cdots,\Phi_k(N)]\\
    \Phi_k(l)&:=\left\{
        \begin{aligned}
    &e^{A_cT(N\theta_k-l)} &l&=1,\cdots,\lfloor N\theta_k\rfloor \\
    &\int_0^{N\theta_k-\lfloor N\theta_k\rfloor} e^{A_c\tau}d\tau B_c & l&=\lfloor N\theta_k\rfloor+1 \\
    &0 & &\text{otherwise}
        \end{aligned}
        \right.
    \end{split}\notag
\end{equation}
Therefore, so as to $\left\|x_{u+a}(t_k)-x_u(t_k)\right\|\geq h_k$, the parameter $\kappa_k$ should be 
\begin{equation}
    \kappa_k\geq\frac{h_k+\left\|\bar{A}_k\Delta\tilde{x}[k]+\Phi_k\xi_k\right\|_2}{\left\|\Phi_k\eta\right\|_2}\notag
\end{equation}
for each $k$.\par
Sufficient condition to exist the parameters $\kappa_k$, $\eta$, $\xi_k$ is as follows.
\begin{enumerate}
    \renewcommand{\labelenumi}{(\alph{enumi})}
      \setlength{\topsep}{0pt}
      \setlength{\partopsep}{0pt}
      \setlength{\itemsep}{0pt}
      \setlength{\parsep}{0pt}
      \setlength{\parskip}{1pt plus 1pt minus 1pt}
    \item $\ker \tilde{C}\tilde{B}_N\neq\{0\}$
    \item For $\{t_k\}_{k=0}^{\infty}$, $\ker \tilde{C}\tilde{B}_N\nsubseteq\ker\Phi_k$
    \item $\im \tilde{C}\tilde{A} \subset \im \tilde{C}\tilde{B}_N$
\end{enumerate}
If $B$ has full column rank and (a) is satisfied, then we can construct the time sequence $\{t_k\}_{k=0}^{\infty}$ which satisfies (b). In particular, we obtain it which is of the form 
\begin{equation}
    \begin{split}
        t_k&=T(Nk+l^*)\\
        &=Tn_k
    \end{split}\label{eq:re:time}
\end{equation}
for each $k$ where $l^*\in\mathbb{N}$. In this section, we assume $B$ has full column rank, both (a) and (c) is satisfied and $l^*$ is given. At this time, if the sequence $\{h_k\}_{k=0}^{\infty}$ is given, then we can calculate the attack $\{a[k]\}_{k=0}^{\infty}$ at each sampling time of sensor. In the sequel, the sequence $\{h_k\}_{k=0}^{\infty}$ is called the attack parameter of the attack.\par
\textbf{Remark}: If the attack by \eqref{eq:re:atk} is statically quantized, it is $\epsilon$-stealth with respect to $\epsilon$ which satisfies \eqref{eq:re:staticeps}.
\begin{equation}
 \epsilon
 \geq \frac{\left\|\sum\limits_{k=0}^\infty
       \abs(\tilde{C}\tilde{A}^k\tilde{B}_N)\right\|_\infty d}{2}
\label{eq:re:staticeps}
\end{equation}
The right side of this inequality is same as \eqref{eq:dq:staticeps} where $A\rightarrow\tilde{A}$, $B\rightarrow\tilde{B}_N$, $C\rightarrow\tilde{C}$.

\subsection{Proposed method 3}\label{se:dqzsa}
In this subsection, we propose the method modifies zero stealthy attack by using the dynamic quantizer before implementation the attack. It is assumed $CB$ is non-singular. Since it is also assumed that $A-B(CB)^{-1}CA$ is stable in this section, the dynamic quantizer in \ref{se:dq} can be utilized.\par 
The method in this subsection generates the quantized attack $\{b[k]\}_{k=0}^{\infty}$ as follows from the attack $\{a[k]\}_{k=0}^{\infty}$ in previous subsection.
\begin{equation*}
    \begin{split}
        \xi[k+1]&=A\xi[k]+B(b[k]-a[k])\\
        b[k]&=q\left(-(CB)^{-1}CA\xi[k]+a[k]\right)
    \end{split}
\end{equation*}
The above equation is updated at each sampling time of the input, not the output. According to \eqref{eq:dq:erroropt}, following inequality is held for every $k$.
\begin{equation*}
    \left\|Cx_b[k]-Cx_a[k]\right\|_\infty\leq\frac{\left\|\sum\limits_{k=0}^\infty\abs(CB)\right\|_\infty d}{2}
\end{equation*}
This inequality also implies 
\begin{equation*}
\begin{split}
        \left\|y_b[k]-y_a[k]\right\|_\infty&=\left\|Cx_b[Nk]-Cx_a[Nk]\right\|_\infty\\&\leq\frac{\left\|\sum\limits_{k=0}^\infty\abs(CB)\right\|_\infty d}{2}.
\end{split}
\end{equation*}
The attack by the above method is characterized by the following theorem. The matrix $\bar{A}$ is given by
\begin{equation}
    \bar{A}:=\begin{bmatrix}
    A & -B(CB)^{-1}CA \\
    O & A-B(CB)^{-1}CA
    \end{bmatrix}.\notag
\end{equation}
\begin{theo}
The sequence $\{H_k\}_{k=0}^{\infty}$ and quantization width $d$ are given. Consider zero stealthy attack $\{a[k]\}_{k=0}^{\infty}$ in \ref{se:zsa} whose attack parameter is $h_k:=H_k+\frac{\sqrt{n}}{2}\alpha_k$ is modified by the dynamic quantizer in \ref{se:dq}, let this attack be $\{b[k]\}_{k=0}^{\infty}$. This attack is $\epsilon$-stealth for $\epsilon$ satisfies \eqref{eq:re:eps} and $\{H_k\}_{k=0}^{\infty}$-disruptive.
\begin{equation}
    \epsilon\geq\frac{\left\|\abs(CB)\right\|_\infty d}{2}\label{eq:re:eps}
\end{equation}
Here,
\begin{equation}
    \alpha_k:=\left\|\sum\limits_{l=0}^{n_k-1}\abs\biggm(\begin{bmatrix}
    I & O
    \end{bmatrix}\bar{A}^{l}\begin{bmatrix}
    B \\
    B
    \end{bmatrix}\biggm)\right\|_\infty.\label{eq:re:alpha}
\end{equation}
\end{theo}
\begin{proof}
According to the triangle inequality, the output error satisfies
\begin{equation}
\left\|y_{v+b}[k]-y_v[k]\right\|_\infty\leq\left\|y_{v+b}[k]-y_{v+a}[k]\right\|_\infty+\left\| y_{v+a}[k]-y_v[k]\right\|_\infty\notag
\end{equation}
for each $k$. The second term of the right side is always 0, because zero stealthy attack $\{a[k]\}_{k=0}^\infty$ holds $y_{v+a}[k]=y_v[k]$ for every $k$. From linearity, the first term of the right side coincides with $\left\| y_b[k]-y_a[k]\right\|_\infty$. Since $a[k]$ is dynamically quantized, 
\begin{equation}
\sup\limits_k\left\| y_b[k]-y_a[k]\right\|_\infty\leq\left\|\abs(CB)\right\|_\infty\frac{d}{2}.\notag
\end{equation}
So if $\epsilon\geq\left\|\abs(CB)\right\|_\infty \frac{d}{2}$, $\sup\limits_{v,k}\left\| y_{v+b}[k]-y_v[k]\right\|_\infty\leq\epsilon$ is held. It means the attack $\{b[k]\}_{k=0}^\infty$ is $\epsilon$-stealth with respect to $\epsilon$ which satisfies \eqref{eq:re:eps}.\par
Next, consider the state difference. According to the triangle inequality, the state difference satisfies
\begin{equation}
\left\| x_{v+b}[k]-x_v[k]\right\|_2\geq\left\| x_{v+a}[k]-x_v[k]\right\|_2-\left\| x_{v+b}[k]-x_{v+a}[k]\right\|_2\label{eq:re:statediff}
\end{equation}
for each $k$. From linearity, the second term of the right side is equal to $x_b[k]-x_a[k]$. Then the states of the plant and the dynamic quantizer obey following state equation.
\renewcommand{\arraystretch}{0.9}%%%
\begin{equation}
\begin{bmatrix}
x_{b}[k+1] \\
\xi[k+1]\\
x_{a}[k+1]
\end{bmatrix}\hskip-3pt=\hskip-3pt\left[\begin{array}{ccc}
A&O&O\\
O&A&O\\
O&O&A 
\end{array}\right]\hskip-5pt\begin{bmatrix}
x_{b}[k] \\
\xi[k]\\
x_{a}[k]
\end{bmatrix}+\begin{bmatrix}
Bb[k] \\
B(b[k]-a[k])\\
Ba[k]
\end{bmatrix}\notag
\end{equation}
If we define
\begin{equation}
w_q[k]:=q(-(CB)^{-1}CA\xi[k]+a[k])-\{-(CB)^{-1}CA\xi[k]+a[k]\},\notag
\end{equation}
then the quantized attack is expressed as $b[k]=a[k]+w_q[k]-(CB)^{-1}CA\xi[k]$. Note that $\left\|w_q[k]\right\|_\infty\leq d/2$.\par
By using this notation, the above equation is 
\begin{equation}
\begin{bmatrix}
x_{b}[k+1] \\
\xi[k+1]\\
x_{a}[k+1]
\end{bmatrix}\hskip-3pt=\hskip-3pt\left[\begin{array}{@{\hskip-1pt}c|c@{\hskip-1pt}}
\raisebox{-0.5em}{\mbox{\LARGE $\bar{A}$}} & \begin{matrix}
O \\ O
\end{matrix}
\\
\hline
 \begin{matrix}
O & O
\end{matrix} & A
\end{array}\right]\hskip-5pt\begin{bmatrix}
x_{b}[k] \\
\xi[k]\\
x_{a}[k]
\end{bmatrix}+\begin{bmatrix}
B(a[k]+w_q[k]) \\
Bw_q[k]\\
Ba[k]
\end{bmatrix}.\notag
\end{equation}
\renewcommand{\arraystretch}{1}%%%
Applying $x_{b}[k]-x_a[k]=[I~O~-I][x_{b}[k]~\xi[k]\ x_{a}[k]]^T$ and $\xi[0]=0$, the state difference is
\begin{equation}
x_{b}[k]-x_a[k]=\sum\limits_{l=0}^{k-1}\begin{bmatrix}
I & O
\end{bmatrix}\bar{A}^{l}\begin{bmatrix}
B \\
B
\end{bmatrix}w_q[k-l].\notag
\end{equation}
At the time $n_k$,
\begin{equation*}
    \left\|x_{b}[n_k]-x_a[n_k]\right\|_\infty\leq\left\|\sum\limits_{l=0}^{n_k-1}\abs\left(\begin{bmatrix}
    I & O
    \end{bmatrix}\bar{A}^l\begin{bmatrix}
    B \\
    B
    \end{bmatrix}\right)\right\|_\infty\frac{d}{2}\notag   
\end{equation*}
is held \cite{dquant}. Then, the square norm of the state difference satisfies
\begin{equation*}
    \left\| x_{b}[n_k]-x_a[n_k]\right\|_2\\\leq\left\|\sum\limits_{l=0}^{n_k-1}\abs\left(\begin{bmatrix}
    I & O
    \end{bmatrix}\bar{A}^l\begin{bmatrix}
    B \\
    B
    \end{bmatrix}\right)\right\|_\infty\frac{\sqrt{n}d}{2}.\notag  
\end{equation*}
Let the attack parameter of the attack be $\{h_k\}_{k=0}^\infty$, then the first term of \eqref{eq:re:statediff} is equal or greater than $h_k$. Therefore, by using $\alpha_k$ satisfies \eqref{eq:re:alpha}, 
\begin{equation}
\left\| x_{v+b}[n_k]-x_{v}[n_k]\right\|_2\geq h_k-\frac{\sqrt{n}d}{2}\alpha_k\notag
\end{equation}
is held. If $h_k=H_k+\frac{\sqrt{n}d}{2}\alpha_k$, the attack $\{b[k]\}_{k=0}^\infty$ is $\{H_k\}_{k=0}^\infty$-disruptive.
\end{proof}
\textbf{Remark}: By the method in \ref{se:dqzda}, the parameters of the dynamic quantizer and its optimal output error vary depending on the number of unstable zeros the system has and their values. The method in this subsection is independent of such influences. This means the attacker has advantages when the plant has input redundancy, which is an intuitive result. 
\subsection{Proposed method 4}\label{se:search}
In this subsection, we propose the method directly search the quantized attack $\{b[k]\}_{k=0}^{\infty}$ at each sampling time. This is a lattice searching problem under some constraints. If the state difference $\Delta\tilde{x}[k]:=\tilde{x}_{v+b}[k]-\tilde{x}_v[k]$ is given, the output error at next step $\Delta y[k+1]:=y_{v+b}[k+1]-y_v[k+1]$ is 
\begin{equation}
\Delta \tilde{y}[k+1]=\tilde{C}\tilde{A}\Delta\tilde{x}[k]+\tilde{C}\tilde{B}_N\begin{bmatrix}
b[kN] \\
\vdots \\
b[(k+1)N-1]
\end{bmatrix}.\notag
\end{equation}
For given $\epsilon$, if $\left\|\Delta y[k+1]\right\|_\infty\leq\epsilon$ for every $k\geq0$, then the attack is $\epsilon$-stealth. This condition is equivalent to following inequality. 
\begin{equation}
\left\|\frac{\tilde{C}\tilde{A}}{d}\Delta\tilde{x}[k]+\tilde{C}\tilde{B}_N\begin{bmatrix}
b[kN] \\
\vdots \\
b[(k+1)N-1]
\end{bmatrix}\right\|_\infty\leq\frac{\epsilon}{d}\label{eq:re:stealth}
\end{equation}
$\frac{b[k]}{d}$ is an integer vector. Hence, so as to satisfy \eqref{eq:re:stealth}, we should the integer vector $v\in\mathbb{Z}^{mN}$ such that
\begin{equation}
\left\|\frac{\tilde{C}\tilde{A}}{d}\Delta\tilde{x}[k]+\tilde{C}\tilde{B}_Nv\right\|_\infty\leq\frac{\epsilon}{d}.\notag
\end{equation}\par
Next, consider the condition for $\{H_k\}_{k=0}^{\infty}$-disruptive. At time $n_k$, the state difference is
\begin{equation}
x_{v+b}[n_k]-x_v[n_k]=A^{k^*}\Delta\tilde{x}[k]+\tilde{B}_{l^*}\begin{bmatrix}
b[kN] \\
\vdots \\
b[(kN+l^*-1]
\end{bmatrix}.\notag
\end{equation}
If we search an integer vector $v_1\in\mathbb{Z}^{mk^*}$ such that 
\begin{equation}
\left\|\frac{A^{k^*}}{d}\Delta\tilde{x}[k]+\tilde{B}_{k^*}v_1\right\|_2\geq\frac{H_k}{d}\notag
\end{equation}
and let $[b[kN]^T\cdots b[kN+k^*-1]^T]^T=v_1d$, then the attack is $\{H_k\}_{k=0}^\infty$-disruptive. Hence, the following theorem is held.
\begin{theo}
It is assumed that the sequence $\{H_k\}_{k=0}^\infty$ and the quantized width $d$ is given. Consider the integer vectors $v_1\in\mathbb{Z}^{ml^*}$ and $v_2\in\mathbb{Z}^{m(N-l^*)}$ which satisfy \eqref{eq:re:cri}. If $[a[kN]^T\cdots a[(k+1)N-1]^T]=d[v_1^T,v_2^T]$, then $b[k]=a[k]$ for every $k$ and the attack is $\epsilon$-stealthy with respect to the $\epsilon$ which satisfies \eqref{eq:re:epsopt} and $\{H_k\}_{k=0}^{\infty}$-disruptive.
\begin{equation}
    \begin{split}
        &\left\|\frac{\tilde{C}\tilde{A}}{d}\Delta\tilde{x}[k]+\tilde{C}\tilde{B}_Nv\right\|_\infty\leq\frac{\epsilon}{d}\\
        &\left\|\frac{A^{k^*}}{d}\Delta\tilde{x}[k]+\tilde{B}_{k^*}v_1\right\|_2\geq\frac{H_k}{d}
    \end{split}\label{eq:re:cri}
\end{equation}
\begin{equation}
   \epsilon\geq\sup\limits_k\epsilon_k\label{eq:re:epsopt}
\end{equation}
Here,
\begin{equation}
\begin{split}
    \epsilon_k:=\sup\limits_{x\in\mathbb{R}^n}\inf_{\substack{v_1\in V_k(x)\\ v_2\in\mathbb{Z}^{m(N-l^*)}}}\left\|\frac{\tilde{C}\tilde{A}}{d}x+\tilde{C}\tilde{B}_N\begin{bmatrix}
    v_1 \\
    v_2 
    \end{bmatrix}\right\|_\infty d\\
    V_k(x):=\biggm\{v\in\mathbb{Z}^{l^*m}\biggm|\left\|\frac{A^{l^*}}{d}x+\tilde{B}_{l^*}v\right\|_2>\frac{H_k}{d}\biggm\}.
\end{split}
\end{equation}
\end{theo}
\textbf{Remark}: The method adopting the dynamic quantizer in \ref{se:dqzsa} calculates the attack by updating a state space equation and solving an equation. On the other hand, the method in this subsection solves the lattice searching problem under the constraints \eqref{eq:re:cri}, which means this type of method costs higher than the method in \ref{se:dqzsa}. However, this method may achieve $\epsilon$-stealthy with respect to lower $\epsilon$. Note that the evaluation of the right side of \eqref{eq:re:epsopt} is the future work.
\subsection{Numerical example}
Consider the following continuous time system for Fig.~\ref{fig:pr:sys}.
\begin{equation}
\begin{split}
\dot{x}(t)&=\begin{bmatrix}
-5 & 1 \\
0 & -2
\end{bmatrix}x(t)+\begin{bmatrix}
0 \\ 1
\end{bmatrix}(v(t)+b(t))\\
y(t)&=\begin{bmatrix}
1 & 1
\end{bmatrix}x(t)
\end{split}\notag
\end{equation}
The sampling period of the control input is $T=0.1[s]$ and $N=2$. The initial state $x_0=0$. It is assumed $u[k]=\sin{0.1\pi k}+2\cos{0.05\pi k}$. The quantization width $d=1$ and $l^*=1$. Let the sequence $\{H_k\}_{k=0}^\infty$ be $H_k=0.01\times1.2^k$ for each $k$.\par
First, the results are depicted from the statically quantized zero stealthy attack in \ref{se:zsa}. Fig.~\ref{fig:re:responseredsta} shows the inter-sample responses under the attack and without the attack. It also shows the system output under the attack at each sampling time $2kT_s~(k=0,1,\ldots)$. In this case, the right side of \eqref{eq:re:staticeps} is $\left\|\sum_{k=0}^\infty\abs(\tilde{C}\tilde{A}^k\tilde{B}_N)\right\|_\infty\frac{d}{2}=0.300$. Fig.~\ref{fig:re:stazsa} shows the control input and sum of the input and the attack.\par
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/responsesredsta.eps}
 \caption{System responses under static quantized zero stealthy attack.  \label{fig:re:responseredsta}}
\end{figure}
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/ua_stazsa.eps}
 \caption{Control inputs and inputs contaminated by static quantized zero stealthy attack.  \label{fig:re:stazsa}}
\end{figure}\par
Next, the results are depicted from the dynamically quantized zero stealthy attack, which is explained in \ref{se:dqzsa}. Fig.~\ref{fig:re:responsered1} shows the inter-sample responses under the attack and without the attack. It also shows the system output under the attack at each sampling time $2kT_s~(k=0,1,\ldots)$. Fig.~\ref{fig:re:y_1} shows the difference between the output under the attack and attack-free output. Though the inter-sample response under the attack is largely deviated, the sampled outputs are closer to the attack-free ones. In fact, the difference between attacked/original outputs are not greater than $\epsilon=\left\|\abs(CB)\right\|_\infty\frac{d}{2}=0.0473$. Fig.~\ref{fig:re:xnorm} is $H_k$ and $\left\|x_{v+b}[n_k]-x_v[n_k]\right\|_2$ at each $k$. It means always $\left\|x_{v+b}[n_k]-x_v[n_k]\right\|_2\geq H_k$. Therefore, the attack is $\{H_k\}_{k=0}^{\infty}$-disruptive. Fig.~\ref{fig:re:dqzsa} shows the control input and sum of the input and the attack.\par
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/responsered1.eps}
 \caption{System response under quantized zero-stealthy attack.  \label{fig:re:responsered1}}
\end{figure} 
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/y_1.eps}
 \caption{Difference of outputs of system under quantized zero-stealthy attack.  \label{fig:re:y_1}}
\end{figure}
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/xnorm.eps}
 \caption{Series $\{H_k\}_{k=0}^{\infty}$ and norm of states difference $\left\|x_{v+b}[n_k]-x_v[n_k]\right\|_2$ under quantized zero-stealthy attack. \label{fig:re:xnorm}}
\end{figure}
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/ua_dqzsa.eps}
 \caption{Control inputs and inputs contaminated by quantized zero stealthy attack. \label{fig:re:dqzsa}}
\end{figure} \par
Next, the results are depicted from the attack method by searching the integer vector in \ref{se:search}. Similarly, Fig.~\ref{fig:re:responsered2} shows the inter-sample responses under the attack and without the attack. It also shows the system output under the attack at each sampling time $2kT_s~(k=0,1,\ldots)$. Fig.~\ref{fig:re:y_2} shows the difference between the output under the attack and attack-free output. Here, $\epsilon=\left\|\abs(CB)\right\|_\infty\frac{d}{8}$. For this $\epsilon$, though the attack method in \ref{se:dqzsa} may not hold $\epsilon$-stealthy property, this type of method is $\epsilon$-stealthy. Fig.~\ref{fig:re:xnorm2} shows this attack is $\{H_k\}_{k=0}^{\infty}$-disruptive. Fig.~\ref{fig:re:epsatk} shows the control input and sum of the input and the attack. Note that the input signal under the attack largely fluctuate compared with the previous two methods. In this case, $\epsilon$ is small so the number of lattices $[v_1^T,v_2]^T$ which satisfy \eqref{eq:re:cri} decrease. Then the attacker results in picking a lattice where $v_1$ is larger than it needs to be.
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/responsered2.eps}
 \caption{System responses under integer attack.  \label{fig:re:responsered2}}
\end{figure} 
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/y_2.eps}
 \caption{Difference of outputs of system under integer attack.  \label{fig:re:y_2}}
\end{figure}
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/xnorm2.eps}
 \caption{Series $\{H_k\}_{k=0}^{\infty}$ and norm of states difference $\left\|x_{v+b}[n_k]-x_v[n_k]\right\|_2$ under integer attack. \label{fig:re:xnorm2}}
\end{figure}
\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{workspace/picture/ua_epsatk.eps}
 \caption{Control inputs and inputs contaminated by integer attack.   \label{fig:re:epsatk}}
\end{figure} 

==> workspace/introduction.tex <==
\section{Introduction}\label{ch:introduction}

Recent advances in communication technology are
enabling various cyber-physical systems (CPSs)
to be further connected by networks, leading to 
enhancements in efficiency and flexibility for
their operation and control. Application domains
where such changes have brought significant 
progress include large-scale plants, smart grids, 
and traffic networks. It is however inevitable that 
along with the increase in networks,
cyber-security issues have gained much more attention. 
Some of the major incidents include 
the attacks against nuclear research facilities in Iran
\cite{Farwell2011StuxnetAT}, 
power grids in Ukraine \cite{ukraine}, and 
sewage systems in Australia \cite{Slay2007LessonsLF}.

To maintain the defense in depth for security and safety
of such CPSs, it is of critical
importance to strengthen security methods from the
perspective of systems control
to complement conventional security methods based on 
information technologies \cite{FerTei:22,IshZhu:22}.
In particular, malicious cyber attacks against CPSs
may have physical consequences, which can 
potentially result in damages in control devices and
facilities. 

In the systems control area, recent research has studied
analyses on impacts of such attacks,
detection techniques, as well as resilient control methods.
Representative classes of attacks that may lead to manipulating
vulnerable physical plants include those of replay attacks, 
Denial-of-Service (DoS) attacks, and 
false-data injection (FDI) attacks;
see, for example, \cite{MoKimBra:12,contsec,TeiShaSan:15}
and the references therein.

The focus of this paper is on the class of FDI attacks
known as the zero dynamics attacks \cite{ParShiLee:19,TeiShaSan:15}. 
An attacker who is aware of the system dynamics may
modify the control signals in such a way that the
internal states of the system are manipulated by the
attacker and can diverge. 
They can be generated by taking advantage of 
system zeros and, in particular, the unstable ones. 
The difficulty in dealing with such attacks is that
the behavior of the system output remains the same 
as that without the attacks. Hence, it is hard to detect 
them, e.g.,
by conventional fault detection techniques.

In this paper, we formulate a networked control 
problem in the sampled-data setting, where 
the continuous-time plant is controlled by a digital 
compensator and the control 
input is transmitted over a network channel.
We place particular attention to the role played by 
quantization in the control signals. Note that zero dynamics
attacks normally require the attack signal to be continuous.
Hence, quantization will introduce certain errors
not only in the attacks but also in the system outputs,
which may make it easier to detect the attacks.
In this sense, the security level can be enhanced by 
using quantization and especially when it is coarse. 
Clearly, there will be a certain tradeoff between
the security level and the control performance since
coarse quantization can in general degrade the system
performance. 

It is important to note that sampled-data systems
can introduce vulnerability in the context of zero 
dynamics attacks \cite{ShiBacEun:22}. 
Even if the continuous-time plant
originally has no unstable zero, when discretized,
the socalled sampling zeros will appear and
some of them can be unstable depending on the 
sampling rate \cite{astrom}. Such unstable zeros
can be exploited by the attacker. 

Quantization in networked control has been studied 
from various perspectives in the past two decades;
see, e.g., \cite{IshFra_book:02,NaiFagZamEva:07}.
%A well-known line of studies is related to the 
%level of quantization necessary to stabilize unstable
%systems based on the minimum data rate 
%(e.g., \cite{}) and the coarsest quantizers (e.g., \cite{}).
For systems under DoS attacks, the effects of quantization
have been addressed in \cite{katoDoS,wakaikiDoS,fengDoS}. 
The general implication found there is that using finer 
quantization, which
requires higher data rate for the communication of
control signals, would improve the robustness of the 
system against DoS attacks and vice versa.

To the best of our knowledge, however, 
quantization and their influence on FDI attacks have
not been studied in the literature.
Here, we will provide an analysis on the error in 
the system output caused by quantizing zero dynamics 
attacks as well as their capability to destabilize the
system. Our problem setting is limited to systems under
feedforward control, but 
it will be shown that by taking account of quantization 
effects, attack signals can be generated
resulting in a lower error level in comparison to 
the simple approach of directly quantizing the 
conventional zero dynamics attacks. 
To this end, we propose two quantized attack methods, one
based on dynamic quantizers \cite{dquant,sythdq} and the other
using a modified version of zero dynamics attacks. 
These methods are constructive in that the attacker
can specify the size of tolerable errors in the system
output and generate attack signals accordingly. 


\if0
For networked control systems, 
the control method which considers a quantization 
of signals caused by actuator capabilities and 
limitations of network communication. 
However, the attack methods previously mentioned 
assume the continuous signals. 
Therefore, it is necessary to study on an attack 
method which takes signal quantization effect into account.

In this paper, we consider a sampled-data system 
whose input signals are quantized. If a system 
input is continuous, the zero dynamics attack 
reduces effect on a system output by adjusting 
its initial value. If not, quantization effect 
appears with respect to its width and a system 
state and output are affected. Consequently, 
the attack performance such as the difficulty 
of detection is seemed to be spoiled.

Therefore, we propose the construction methods 
of the attack and analyze its effect, which reduce 
quantization effect on a system output and deviate 
a system state while a system input is quantized. 
In particular, for the cases where a sampled-data 
system has unstable zeros, we propose the two types 
of methods as follows.
\begin{itemize}
    \item the method utilizes a continuous attack signal.
    \item the method directly calculates a quantized attack signal.
\end{itemize}
\fi

The reminder of this paper is organized as follows: 
Section~\ref{ch:problem} describes the networked control 
system, the input quantizer and the class of the attacks. 
In Section~\ref{ch:dq}, we briefly overview 
the approach of dynamic quantizers, which will be used for
attack signal generation in one of the proposed methods.
In Section~\ref{ch:nonmin}, we explain the two methods 
of quantized attacks for a non-minimum phase 
sampled-data systems and analyze their effects. 
In Section~\ref{ch:example}, we illustrate the effectiveness
of our results via a numerical example.  
In Section~\ref{ch:conclusion}, we provide 
concluding remarks. 

\textbf{Notation}: We denote by $\mathbb{R}$, $\mathbb{N}$ and $\mathbb{Z}$ the sets of real numbers, natural numbers and integers respectively. %Moreover, $\mathbb{R}^n$, $\mathbb{R}^{n\times m}$ are $n$ dimensional real vectors and $n$ by $m$ real matrices respectively.
For $d>0$, $d\mathbb{Z}$ is the set of numbers which can be expressed as $dz$ by using an integer $z\in\mathbb{Z}$. 
The space of bounded sequences is denoted by $l_\infty$. 
%Non-negative integers are denoted as $\mathbb{Z}_+$. 
%For a matrix $A:=[A_{ij}]$, $\abs(A):=[|A_{ij}|]$. The $\infty$-norm of the vector $v$ is written as $\left\| v\right\|_\infty=\max_i|v_i|$. Similarly, $\left\| A\right\|_\infty$ is the $\infty$-norm of the matrix $A$, which is induced by vector's $\infty$-norm. 

==> workspace/introduction0.tex <==
\section{Introduction}\label{ch:introduction}

Recently, advances in communication technology and 
computer led cyber-physical system technology to 
be more practical, which improves efficiency and 
flexibility of physical systems by using computers 
to supervise and control. This technology is applied 
to various objects such as large-scale plants, 
smart grid and traffic networks. 
On the other hand, its security problems also gets 
attention. Recent example of incidents include the 
cyber attack on Iran's nuclear plant by the 
Stuxnet and the Ukrainian power grid, the massive 
power blackouts in Brazil and the malfunction of 
sewage system in Australia \cite{Farwell2011StuxnetAT,Brazil,Slay2007LessonsLF,ukraine}. 
These examples reveals the importance of prevention and 
detection of the vulnerabilities of cyber-physical 
systems and the unexpected incidents. 
In particular, necessity of the system control 
security is pointed out in addition to conventional 
security based on information technologies\cite{teixeirabook,ishiibook},

So far, the vulnerabilities of cyber-physical systems 
are discussed from the system control point of view. 
For example, the false data injection attack, 
DoS attack and the replay attack are analyzed. 
Also, it is studied to detect them \cite{FDIs,Mo2010FalseDI,replay,contsec,katoDoS,wakaikiDoS,fengDoS}. 

The zero dynamics attack \cite{zda,revealing} 
is the attack method taking advantage of system zeros. 
In particular, if a system has unstable zeros, 
then this attack is difficult to detect from 
a system output and a system state diverges. 
In general, networked control systems are 
deployed as sampled-data systems, which is 
composed of a continuous time plant and a 
discrete time digital controller. 
In this case, the zeros which do not exist in 
a continuous plant may appear because of 
discretization, which are called discrete 
zeros \cite{astrom}. Because there may exist 
unstable discrete zeros, the zero dynamics attack 
is seemed to be important method for sampled-data 
systems. 

For networked control systems, 
the control method which considers a quantization 
of signals caused by actuator capabilities and 
limitations of network communication. 
However, the attack methods previously mentioned 
assume the continuous signals. 
Therefore, it is necessary to study on an attack 
method which takes signal quantization effect into account.

In this paper, we consider a sampled-data system 
whose input signals are quantized. If a system 
input is continuous, the zero dynamics attack 
reduces effect on a system output by adjusting 
its initial value. If not, quantization effect 
appears with respect to its width and a system 
state and output are affected. Consequently, 
the attack performance such as the difficulty 
of detection is seemed to be spoiled.

Therefore, we propose the construction methods 
of the attack and analyze its effect, which reduce 
quantization effect on a system output and deviate 
a system state while a system input is quantized. 
In particular, for the cases where a sampled-data 
system has unstable zeros, we propose the two types 
of methods as follows.
\begin{itemize}
    \item the method utilizes a continuous attack signal.
    \item the method directly calculates a quantized attack signal.
\end{itemize}

The reminder of this paper is organized as follows: 
Section~\ref{ch:problem} describes the system considered 
in this paper, the input quantizer and the conditions 
of the attack. In Section~\ref{ch:dq}, we briefly overview 
the approach of dynamic quantizers, which is used to 
adjust a continuous valued attack. 
In Section~\ref{ch:nonmin}, we explain the methods 
of quantized attacks for a non-minimum phase 
sampled-data systems and analyze their effects. 
In Section~\ref{ch:example}, we illustrate our
results via a numerical example.  
In Section~\ref{ch:conclusion}, we provide 
concludiong remarks. 

\textbf{Notation}: We denote by $\mathbb{R}$, $\mathbb{N}$ and $\mathbb{Z}$ the sets of real numbers, natural numbers and integers respectively. Moreover, $\mathbb{R}^n$, $\mathbb{R}^{n\times m}$ are $n$ dimensional real vectors and $n$ by $m$ real matrices respectively. For $d>0$, $d\mathbb{Z}$ is the set of numbers which can be expressed as $dz$ by using an integer $z\in\mathbb{Z}$. The set of finite sequences are denoted as $l_\infty$. 
%Non-negative integers are denoted as $\mathbb{Z}_+$. 
%For a matrix $A:=[A_{ij}]$, $\abs(A):=[|A_{ij}|]$. The $\infty$-norm of the vector $v$ is written as $\left\| v\right\|_\infty=\max_i|v_i|$. Similarly, $\left\| A\right\|_\infty$ is the $\infty$-norm of the matrix $A$, which is induced by vector's $\infty$-norm. 

==> workspace/nonmin.tex <==
\section{Quantized attacks for non-minimum phase systems}\label{ch:nonmin}
In this section, we discuss quantized attacks for the case when the sampled-data system \eqref{eq:pr:csys} has unstable zeros. Concretely, we consider three types of methods as follows:

(i)~The first method is simple, where zero dynamics attacks as described in Section~II-C are generated and quantized directly using the static quantizer.\par
(ii)~The second approach employs the dynamic quantizer outlined above to modify the zero dynamics attacks in real values. We can show that this method can achieve smaller output error than statically quantizing the zero dynamics attacks as in the first method. However, it is affected by the number of unstable zeros and their values. \par
(iii)~The third method quantizes attack signals which are slightly different from the conventional zero dynamics attacks and may induce small but bounded influence on the system output. This signal can be constructed without the influence of unstable zeros. Moreover, as we will see in the analysis as well as numerical examples, this method is capable to outperform the other two methods in terms of the output error.\par
In this section, we look at these three attack methods and analyze the resulting output errors. 
\subsection{Quantized attack method 1 via static quantization}\label{se:sqzda}
We start with the simplest quantization approach where the attack signal $a[k]$ generated by \eqref{eq:pr:zda} is directly 
quantized in a static manner. That is, the attack
signal $b[k]$ to be injected to the quantized control input $v[k]$ 
in Fig.~1 is given by
\begin{equation}
    b[k] = q(a[k]).
    \label{eq:no:bqa}
\end{equation} 
For this method, we obtain the following result.
%Regarding the quantized attack $\{b[k]\}_{k=0}^{\infty}$ 
%which is calculated by \eqref{eq:pr:zda} and the static 
%quantizer, we obtain the following result.
\begin{prop}
For the quantized networked system under attacks in Fig.~\ref{fig:pr:sys}, suppose that the quantization width $d$ is given and the scalar $\epsilon$ satisfies
\begin{equation}
    \epsilon>\frac{1}{2}\sum\limits_{k=0}^\infty\left|CA^kB\right|d.\label{eq:no:staticeps}
\end{equation}
Moreover, suppose that the attack signal generated by \eqref{eq:pr:zda} is statically quantized as in \eqref{eq:no:bqa}. Then, for any sequence $\{H_k\}_{k=0}^{\infty}$, there exists a quantized attack signal $\{b[k]\}_{k=0}^{\infty}$ that is $\epsilon$-stealthy and $\{H_k\}_{k=0}^{\infty}$-disruptive.
\end{prop}
\begin{sketchofproof}
First, we can upper bound the output error as
\begin{multline*}
    \left|y_{v+b}[k]-y_v[k]\right|\\\leq\left|y_{v+b}[k]-y_{v+a}[k]\right|+\left|y_{v+a}[k]-y_v[k]\right|.
\end{multline*}
The first term on the right-hand side is less than or equal to $\frac{1}{2}\sum_{k=0}^\infty\left|CA^kB\right|d$ from \eqref{eq:dq:staticeps}. By Lemma.~1 and \eqref{eq:no:staticeps}, we can choose the attack signal $\{a[k]\}_{k=0}^{\infty}$ which is $\left(\epsilon-\frac{1}{2}\sum_{k=0}^\infty\left|CA^kB\right|d\right)$-stealthy. Then, the right-hand side of the above inequality is less than or equal to $\epsilon$. Therefore the attack $\{b[k]\}_{k=0}^{\infty}$ is $\epsilon$-stealthy.\par
Next, we look at the difference in states. We have
\begin{align*}
  &\left\| x_{v+b}[k]-x_v[k]\right\|_2\\
   &~~\geq \left\| x_{v+a}[k]-x_v[k]\right\|_2
       - \left\| x_{v+b}[k]-x_{v+a}[k]\right\|_2.
\end{align*}
On the right-hand side, the first term diverges as $k\rightarrow\infty$. The second term on the right-hand side coincides with the state which is driven by the quantization error; since the quantization error is bounded and the system \eqref{eq:pr:dsys} is stable, this term is also bounded. It means that $\left\| x_{v+b}[k]-x_v[k]\right\|_2$ diverges as $k\rightarrow\infty$. Therefore, we conclude that the attack $\{b[k]\}_{k=0}^{\infty}$ is $\{H_k\}_{k=0}^{\infty}$-disruptive.
\end{sketchofproof}
\subsection{Quantized attack method 2 via dynamic quantization}\label{se:dqzda}
In this subsection, we propose a method which modifies the continuous zero dynamics attacks in Section \ref{ch:problem} by using dynamic quantization from the previous section. This method adopts dynamic quantizer based on serial decomposition in Section \ref{se:dqseri}. \par
Specifically, we apply \eqref{eq:dq:dqseri} to generate attack signals after obtaining the serial decompositions $P_s$, $P_u$ of the system \eqref{eq:pr:dsys} satisfying conditions outlined there. The effects to output signals caused by this attack is determined by the choices of $P_s$, $P_u$. As we discussed earlier, while this method can be utilized for systems with any number of unstable zeros, the optimal value for the output error is known only for the case of one unstable zero. The following theorem is the first main result of this paper stating that dynamic quantizer can be efficient in reducing the error due to quantized attacks. 
\begin{theo}\label{theo:dqzda}
For the quantized networked system under attacks in Fig.~\ref{fig:pr:sys}, suppose that the plant is decomposed serially as described in Section \ref{se:dqseri} and $\epsilon$ satisfies
\begin{equation}
    \epsilon>\frac{1}{2}\left\|P_u\right\|_{i\infty}\left|C_sB_s\right|d,\label{eq:no:eps}
\end{equation}
where $B_s$ and $C_s$ are the system matrices of $P_s$. Then, for any sequence $\{H_k\}_{k=0}^\infty$, there exists a quantized attack signal $\{b[k]\}_{k=0}^\infty$ generated by \eqref{eq:pr:zda} and dynamic quantization that is $\epsilon$-stealthy and $\{H_k\}_{k=0}^\infty$-disruptive.
\end{theo}\par
\begin{proof}
By Lemma \ref{lem:zda}, we can construct the attack signal $\{a[k]\}_{k=0}^{\infty}$ such that it is $\left(\epsilon-\frac{1}{2}\left\|P_u\right\|_{i\infty}\left|C_sB_s\right|d\right)$-stealthy and $\left\|x_{u+a}[k]-x_u[k]\right\|_2$ diverges. Consider the attack $\{b[k]\}_{k=0}^{\infty}$ which is made from $\{a[k]\}_{k=0}^{\infty}$ and the dynamic quantizer in Section \ref{se:dqseri}. We verify that this attack satisfies both $\epsilon$-stealthy and $\{H_k\}_{k=0}^{\infty}$-disruptive properties.\par
We can upper bound the output error as
\begin{align}
  & |y_{v+b}[k]-y_v[k]|\\
  &~~~\leq|y_{v+b}[k]-y_{v+a}[k]|
          +| y_{v+a}[k]-y_v[k]|\label{eq:no:ineqy}
\end{align}
for every $k$. Since the system is linear, the first term on the right-hand side coincides with $|y_b[k]-y_a[k]|$. By the bound on the output error \eqref{eq:dq:dqserierroropt} for the dynamic quantizer, this term can be bounded as
\begin{equation}
    \sup\limits_k|y_b[k]-y_a[k]|\leq\frac{1}{2}\left\|P_u\right\|_{i\infty}|C_sB_s|d.\notag
\end{equation}
By the construction of $\{a[k]\}_{k=0}^{\infty}$, the second term on the right-hand side of \eqref{eq:no:ineqy} satisfies the following inequality:
\begin{equation}
    \sup\limits_k|y_{v+a}[k]-y_v[k]|\leq\epsilon-\frac{1}{2}\left\|P_u\right\|_{i\infty}|C_sB_s|d.\notag
\end{equation}
Hence, from \eqref{eq:no:ineqy}, we have $\sup_k| y_{v+b}[k]-y_v[k]|\leq\epsilon$. Consequently, the attack $\{b[k]\}_{k=0}^\infty$ is $\epsilon$-stealthy.\par
Next, we look at the difference in states. We have
\begin{multline}
    \left\| x_{v+b}[k]-x_v[k]\right\|_2\\\geq\left\| x_{v+a}[k]-x_v[k]\right\|_2-\left\| x_{v+b}[k]-x_{v+a}[k]\right\|_2.\label{eq:no:statediff}
\end{multline}
Because of the choice of $\{a[k]\}_{k=0}^{\infty}$, the first term on the right-hand side diverges as $k\rightarrow\infty$. Since the system is linear, it follows that $x_{v+b}[k]-x_{v+a}[k]=x_b[k]-x_a[k]$. The state-space equation of the plant and the dynamic quantizer can be written as
\begin{equation}
\begin{bmatrix}
x_{b}[k+1] \\
\xi[k+1]\\
x_{a}[k+1]
\end{bmatrix}\hskip-3pt=\hskip-3pt\left[\begin{array}{@{\hskip-1pt}c@{\hskip1pt}c@{\hskip1pt}c@{\hskip-1pt}}
A&O&O\\
O&A_s&O\\
O&O&A 
\end{array}\right]\hskip-5pt\begin{bmatrix}
x_{b}[k] \\
\xi[k]\\
x_{a}[k]
\end{bmatrix}\hskip-2pt+\hskip-2pt\begin{bmatrix}
Bb[k] \\
B_s(b[k]-a[k])\\
Ba[k]
\end{bmatrix}.\label{eq:no:xbxixa}
\end{equation}
Let $w_q[k]$ be
\begin{equation*}
        w_q[k]:=q\left(-\frac{C_sA_s}{C_sB_s}\xi[k]+a[k]\right)-\left\{-\frac{C_sA_s}{C_sB_s}\xi[k]+a[k]\right\}.
\end{equation*}
Then, the quantized attack is expressed as $b[k]=a[k]+w_q[k]-\frac{C_sA_s}{C_sB_s}\xi[k]$. Note that $\left\|w_q[k]\right\|_\infty\leq d/2$. Also, let the system matrix $\bar{A}$ be
\begin{equation*}
    \bar{A}:=\begin{bmatrix}
    A & -\frac{BC_sA_s}{C_sB_s} \\
    O & A_s-\frac{B_sC_sA_s}{C_sB_s}
    \end{bmatrix}.
\end{equation*}
\quad Then, the state-space equation in \eqref{eq:no:xbxixa} can be rewritten into 
\begin{equation}
\begin{bmatrix}
x_{b}[k+1] \\
\xi[k+1]\\
x_{a}[k+1]
\end{bmatrix}\hskip-3pt=\hskip-3pt\left[\begin{array}{@{\hskip-1pt}c|c@{\hskip-1pt}}
\raisebox{-0.5em}{\mbox{\LARGE $\bar{A}$}} & \begin{matrix}
O \\ O
\end{matrix}
\\
\hline
 \begin{matrix}
O & O
\end{matrix} & A
\end{array}\right]\hskip-5pt\begin{bmatrix}
x_{b}[k] \\
\xi[k]\\
x_{a}[k]
\end{bmatrix}+\begin{bmatrix}
B(a[k]+w_q[k]) \\
B_sw_q[k]\\
Ba[k]
\end{bmatrix}.\notag
\end{equation}
Applying $x_{b}[k]-x_a[k]=[I~O~-I][x_{b}[k]~\xi[k]\ x_{a}[k]]^T$ and $\xi[0]=0$ to it, we can obtain the relation
\begin{equation}
x_{b}[k]-x_a[k]=\sum\limits_{l=0}^{k-1}\begin{bmatrix}
I & O
\end{bmatrix}\bar{A}^{l}\begin{bmatrix}
B \\
B_s
\end{bmatrix}w_q[k-l].\notag
\end{equation}
Since the system \eqref{eq:pr:dsys} is stable and the subsystem $P_s$ is minimum phase, the matrix $\bar{A}$ is also stable. Thus, the sequence $x_{b}[k]-x_a[k]$ is bounded, implying that the second term on the right-hand side of \eqref{eq:no:statediff} is bounded. Consequently, $\left\| x_{v+b}[k]-x_v[k]\right\|_2\rightarrow\infty$ as $k\rightarrow\infty$. Therefore, we conclude that the quantized attack signal $\{b[k]\}_{k=0}^\infty$ is $\{H_k\}_{k=0}^{\infty}$-disruptive.
\end{proof}
\subsection{Quantized attack method 3 via $\epsilon$-stealthy approach}\label{se:calc}

The third method employs a continuous attack signal 
which is a slightly modified version of the zero 
dynamics attack in \eqref{eq:pr:zda} and then quantizes 
it directly. 

To this end, for given $\epsilon>0$, let us consider 
the attack signal $\{a[k]\}_{k=0}^{\infty}$ generated by
\begin{equation}
    \begin{split}
        z[k+1]&=\left(A-\frac{BCA}{CB}\right)z[k]+\frac{B}{CB}\epsilon,\\
        a[k]&=-\frac{CA}{CB}z[k]+\frac{\epsilon}{CB},
    \end{split}\label{eq:no:zdag}
\end{equation}
where $z[0]=0$. We can easily show that this system 
is unstable and the state difference difference $x_{u+a}[k]-x_u[k]$ is equal to $z[k]$. 
It means that $y_{u+a}[k]-y_u[k]=Cz[k]$ and this value 
coincides with $\epsilon$ for $k\geq1$. 
Hence, this attack is $\epsilon$-stealthy in the sense of \eqref{eq:pr:estealth} (without quantization).

The system \eqref{eq:no:zdag} motivates us to generate attack
signals using a system which has constant input proportional 
to $\epsilon$ and then to quantize the signal. 
This can be achieved by introducing the following quantized system:
%a quantized version which generates the quantized attack signal $\{b[k]\}_{k=0}^{\infty}$ as
\begin{equation}
 \begin{split}
   z[k+1]&=Az[k]+Bb[k],\\
        b[k]&=q\left(-\frac{CA}{CB}z[k]+\frac{\sign(CB)\epsilon}{CB}-\frac{d}{2}+\Delta\right),
    \end{split}\label{eq:no:dzdag}
\end{equation}
where $\Delta$ is a sufficiently small positive number. \par
Now, we are ready to state our second main result of the paper. 
\begin{theo}\label{theo:2}
For the quantized networked system under attacks in Fig.~\ref{fig:pr:sys}, suppose that $\epsilon$ is taken as $\epsilon \geq |CB|d$. Then, for any sequence $\{H_k\}_{k=0}^{\infty}$, the quantized attack $\{b[k]\}_{k=0}^{\infty}$ generated by \eqref{eq:no:dzdag} is $\left(\epsilon + |CB|\Delta\right)$-stealthy and $\{H_k\}_{k=0}^{\infty}$-disruptive. 
%if the following conditions are satisfied:
%\begin{itemize}
%    \item Consider the Jordan decomposition of $\left(A-\frac{BCA}{CB}\right)=P\Lambda P^{-1}$. Moreover, let the diagonal elements of $\Lambda$ be $\sigma_1,\ldots,\sigma_n$ and $\sigma_l,\ldots,\sigma_n$ be unstable ones. Then at least one of the $l-th$ through the last element of $B':=P^{-1}B$ is not $0$.
%\end{itemize}
\end{theo}
\begin{proof}
It is straightforward to show that by \eqref{eq:no:zdag}, the differences in states and output can be written as $x_{v+b}[k]-x_v[k]=z[k]$ and $y_{v+b}[k]-y_v[k]=Cz[k]$ respectively. Let  
\[
  w[k]:=(-\frac{CA}{CB}z[k]+\frac{\sign(CB)\epsilon}{CB}+\Delta)-b[k]. 
\]
Then, \eqref{eq:no:dzdag} becomes
\begin{multline}
    z[k+1]=\left(A-\frac{BCA}{CB}\right)z[k]\\+B\left(\frac{\sign(CB)\epsilon}{CB}+\Delta-w[k]\right),
\end{multline}
where $0<w[k]\leq d$. Since $z[0]=0$, we have 
\begin{align}
&z[k]\notag\\
&~~= \sum_{l=0}^{k-1}\left(A-\frac{BCA}{CB}\right)^{k-l-1}
   B\left(\frac{\sign(CB)\epsilon}{CB}+\Delta-w[l]\right).
\label{eq:no:zk}
\end{align}
Note that it holds $C\left(A-\frac{BCA}{CB}\right)=0$ and $Cz[k]=\sign(CB)\epsilon+CB\Delta-CBw[k-1]$ for all $k\geq1$. Since $\epsilon\geq|CB|d$, it holds 
\[
  -\left(\epsilon+|CB|\Delta\right)
    \leq|Cz[k]|\leq\epsilon+|CB|\Delta. 
\]
It means that the attack $\{b[k]\}_{k=0}^{\infty}$ is $\left(\epsilon+|CB|\Delta\right)$-stealthy.\par
Next, to establish that $\{b[k]\}_{k=0}^{\infty}$ is $\{H_k\}_{k=0}^{\infty}$-disruptive, we must show that $z[k]$ diverges, which implies that $\left\|x_{v+b}[k]-x_v[k]\right\|_2$ also diverges. Let 
\[
  w'[k]:=\frac{\sign(CB)\epsilon}{CB}+\Delta-w[k].
\] 
Now, based on \eqref{eq:no:zk}, we can rewrite the system of $z[k]$ and
obtain
\begin{equation*}
   z[k+1] = \left(A-\frac{BCA}{CB}\right) z[k] + B w'[k].
\end{equation*}
Since $z[0]=0$, we must make sure that in this system, the input $w'[k]$ enters and excites the unstable mode. \par 
Recall that $\left(A,B\right)$ is controllable, and thus $\left(A-\frac{BCA}{CB}, B\right)$ is also controllable. Hence, it follows that the input $w'[k]$ enters every mode of the system. Finally, we can confirm that $w'[k]$ is not zero at all times. By assumption, $\epsilon\geq|CB|d$, and this implies that $w'[k]\geq\Delta$ at each $k$. Therefore, the state $z[k]$ diverges.
%Next, we look at $z[k]$. The matrix $A-\frac{BCA}{CB}$ can be denoted as $P\Lambda P^{-1}$ by Jordan decomposition. Moreover, we can let the diagonal elements of $\Lambda$ be $\sigma_1,\ldots,\sigma_n$ and $\sigma_l,\ldots,\sigma_n$ be unstable ones.  Since $\epsilon\geq|CB|d$, the new variable $w'[k]:=\frac{\sign(CB)}{CB}\epsilon+\Delta-w[k]$ satisfies $w'[k]\geq\Delta$. Then, \eqref{eq:no:zk} becomes
%\begin{equation}
%    z[k]=\sum_{l=0}^{k-1}P\Lambda^{k-l-1}B'w'[l],\label{eq:no:zk2}
%\end{equation}
%where $B':=P^{-1}B$. Since $\left(A, B\right)$ is controllable, $\left(A-\frac{BCA}{CB}, B\right)$ is also controllable. Therefore, the vector $B'$ has nonzero elements and the last one has index greater than or equal to $l$. Here, we denote this index by $l^*$. Then the state $P^{-1}z[k]$ can be expressed as
%\begin{equation}
%    P^{-1}z[k]=\begin{bmatrix}
%    *\\
%    \vdots\\
%    *\\
%    \sum_{l=0}^{k-1}\sigma_{l^*}^{k-l-1}B_{l^*}'w'[l]\\
%    0\\
%    \vdots\\
%    0
%    \end{bmatrix}.\label{eq:no:zk3}
%\end{equation}
%The square norm of $P^{-1}z[k]$ can be bounded as
%\begin{equation*}
%        \left\|P^{-1}z[k]\right\|_2\leq\left\|P^{-1}\right\|_2\left\|z[k]\right\|_2.
%\end{equation*}
%Then, that of $z[k]$ can be bounded as
%\begin{equation*}
%    \begin{split}
%        \left\|z[k]\right\|_2&\geq\frac{1}{\left\|P^{-1}\right\|_2}\left\|P^{-1}z[k]\right\|_2\\
%        &\geq\frac{1}{\left\|P^{-1}\right\|_2}\left|\sum_{l=0}^{k-1}\sigma_{l^*}^{k-l-1}B_{l^*}'w'[l]\right|\rightarrow\infty.
%    \end{split}
%\end{equation*}
%Hence, $\left\|x_{v+b}[k]-x_v[k]\right\|_2$ also diverges. Consequently, the attack $\{b[k]\}_{k=0}^{\infty}$ is  $\{H_k\}_{k=0}^{\infty}$-disruptive.
\end{proof}
\quad We remark that to achieve the disruptive property, the assumption that $\epsilon \geq|CB|d$ is critical for the quantized attack \eqref{eq:no:dzdag}. This is because the initial state is $z[0]=0$, if $\epsilon<|CB|d$, then $z[k]\equiv0$. This will further result in $b[k]\equiv0$, that is, no quantized attack.\par
Furthermore, compared with the attack approach based on dynamic quantization  of Section \ref{se:dqzda}, the attack \eqref{eq:no:dzdag} of this method has the following feature: If there is only one unstable zero, then the output error is strictly less than 
the right-hand side of \eqref{eq:no:eps}. This holds because with sufficiently small $\Delta$, we have
\begin{equation*}
  \frac{1}{2}\left|CB\right|
    \left(1+|\lambda|\right)d
   >\left|CB\right|\left(d+\Delta\right)
\end{equation*}
where $\lambda$ is the unstable zero with $|\lambda|>1$.
We will confirm this difference between the two methods
in numerical examples presented in the next section.


==> workspace/problem.tex <==
\section{Problem formulation}\label{ch:problem}
In this section, we formulate the problem of quantized FDI attacks studied in this paper.
\subsection{Sampled-data system under quantized input}\label{se:plant}
Consider the feedforward sampled-data control system shown in Fig.~\ref{fig:pr:sys}, where the controller is connected with the plant via a network. The control input is generated by the controller and is quantized before it is sent to the plant over the network. A malicious attacker has access to the network and may modify the input signal though the attack signal must use the same quantization scheme as the controller. 

\begin{figure}[t]
 \vspace*{3mm}
 \centering
  \includegraphics[width=1\linewidth]{workspace/picture/system1.png}
 \vspace*{1mm}
  \caption{Networked sampled-data control system under attack}
  \label{fig:pr:sys}
\end{figure}

In Fig.~\ref{fig:pr:sys},
the plant is a single-input single-output linear time-invariant (LTI) system whose state-space equation is given by
\begin{equation}
    \begin{split}
        \dot{x}(t)&=A_cx(t)+B_c(v(t)+b(t)),\\
        y(t)&=Cx(t),
    \end{split}\label{eq:pr:csys}
\end{equation}
where $x(t)\in\mathbb{R}^n$ is the state, $y(t)\in\mathbb{R}$ is the output, $A_c\in\mathbb{R}^{n\times n}$, $B_c\in\mathbb{R}^{n\times 1}$ and $C\in\mathbb{R}^{1\times n}$ are the system matrices. Moreover, the inputs $v(t)$, $b(t)\in d\mathbb{Z}$ are respectively the quantized signals of the feedforward input $u(t)$ and the attack signal $a(t)$. The specific quantizer used will be introduced later. We assume that the system is stable and controllable, and 
the initial state is $x(0)=x_0$.\par
In this paper, the input $v(t)$ is injected through  the zero-order hold (ZOH) whose sampling period is $T>0$. Denote by $v[k]$ the input calculated by the controller at time $t=kT$. The continuous-time signal applied to the plant is $v(t):=v [k]$ for $t\in[kT,(k+1)T)$. On the other hand, the output $y(t)$ of the plant is sampled at the same rate as the ZOH with sampling period $T$. So the measured output is $y [k] :=y(kT)$. We adopt the notation to write the system state and output of \eqref{eq:pr:csys} driven by input $u(t)$
as $x_u(t)$ and $y_u(t)$ respectively.\par
As the quantizer, we use the uniform quantizer $q:\mathbb{R}\rightarrow d\mathbb{Z}$, whose width is denoted by $d>0$. We use the nearest neighbor quantization towards $-\infty$ \cite{dquant}; it maps $\mu\in\mathbb{R}$ to $q(\mu)$ which is the optimal solution to $\min_{w\in d\mathbb{Z}}(w-\mu)^2$. In Fig.~\ref{fig:pr:sys}, the quantized input is given by
\begin{equation}
   v[k]=q(u[k]).
\label{eqn:vk}
\end{equation}
\subsection{Quantized FDI attacks}
As mentioned above, the adversary is capable to modify the quantized control input $v[k]$ to $v[k]+b[k]$ by injecting the quantized attack signal $b[k]$. It is assumed that the adversary has the full information of the controller and the plant including their dynamics whereas the system operator has no information regarding the attacks. The adversary's objective is to disrupt the operation of the system without being detected by the system operator who may be monitoring the sampled system output $y[k]$. \par
More specifically, the adversary attempts to generate the attack signal $b[k]$ satisfying the following two conditions:\par
(i)~\textbf{$\epsilon$-stealthy condition}: The attack signal $\{b[k]\}_{k=0}^{\infty}$ is said to be $\epsilon$-stealthy for given $\epsilon >0$ if the following inequality is satisfied for every $k$:
\begin{equation}
    \left|y_{v+b}[k]-y_v[k]\right|\leq\epsilon,\label{eq:pr:estealth}
\end{equation}
where $y_v$ is the original output of the system under the input $v$ and $y_{v+b}$ is the output of the attacked system.\par
(ii)~\textbf{$\{H_k\}_{k=0}^{\infty}$-disruptive condition}: Given a sequence of nonnegative numbers $\{H_k\}_{k=0}^{\infty}$, the attack signal $\{b[k]\}_{k=0}^{\infty}$ is said to be  $\{H_k\}_{k=0}^{\infty}$-disruptive if there exists a time sequence $\{t_k\}_{k=0}^{\infty}$ such that the following inequality is satisfied for every $k$:
\begin{equation}
    \left\|x_{v+b}(t_k)-x_v(t_k)\right\|_2\geq H_k.\label{eq:pr:disrupt}
\end{equation}
\quad The problem addressed in the paper can be stated as follows.\par
\textit{Problem}: Let the positive scalar $\epsilon$ and the sequence $\{H_k\}_{k=0}^{\infty}$ of nonnegative numbers be given. Then find the quantized attack signal $\{b[k] \}_{k=0}^{\infty}$ which satisfies both $\epsilon$-stealthy and $\{H_k\}_{k=0}^{\infty}$-disruptive conditions.\par
Particularly, we examine the problem above for the case where the sampled-data system has unstable zeros. \par
If the attacker can inject continuous-valued signals, attack methods satisfying the two conditions above are proposed, which are known as the zero dynamics attacks (ZDA) \cite{TeiShaSan:15,ParShiLee:19}. This type of attacks takes advantage of system zeros. Notably, if the system has unstable zeros, states may diverge and it is difficult to detect such attacks from the output since it will remain almost the same with or without the attack.\par
However, if we place an input quantizer, the system state/output under attacks should be influenced. Consequently, the stealthy and disruptive properties may be lost to some extent. In fact, if the attack signals are statically quantized, then the output receives major influences as we will see later. Hence, quantization may be used as a means to detect attacks on the system. Note that however that quantizing the input would reduce the control performance at the same time. So there is a tradeoff between the attack detection and control performance. The objective of this paper is to demonstrate that different methods for quantization of attack signals can result in different properties and in particular there are ways to reduce the effects caused by quantizers.
\subsection{Zero dynamics attacks}\label{se:zda}
The sampled-data system \eqref{eq:pr:csys} can be expressed as the following discrete-time linear system under ZOH and sampling:
\begin{equation}
    \begin{split}
        x[k+1]&=Ax[k]+B(v[k]+b[k]),\\
        y[k]&=Cx[k],
    \end{split}\label{eq:pr:dsys}
\end{equation}
where $x[k]:=x(kT)$, $A:=e^{A_cT}$ and $B:=\int_0^Te^{A_c\tau}d\tau B_c$. We assume that this system is controllable and the vector product $CB$ is nonsingular, which means the relative degree of this discretized system is $1$; these properties hold for almost any $T>0$ \cite{astrom}. \par
Note that when a continuous-time system is discretized, zeros which do not exist in the original system may appear. These are called the sampling zeros. As mentioned above, regardless of the relative degree of the original system \eqref{eq:pr:csys}, the discretized system \eqref{eq:pr:dsys} has relative degree of $1$ for almost any sampling period $T$. It is known that when $T$ is small, some of them will be unstable \cite{astrom}. Hence, even if the original system has no unstable zero, there is a chance that discretization will introduce some. In such a case, if the input is not quantized, then the zero dynamics attacks proposed in \cite{TeiShaSan:15,ParShiLee:19} can be applied. We note that such attacks can have arbitrarily small effects on the output by taking the initial state accordingly.\par
We summarize how to construct ZDA signals as follows: In this part, we make the following assumption: The system \eqref{eq:pr:dsys} has nonminimum phase zeros. Here, we consider the case where the inputs are not quantized, i.e., $v[k]=u[k]$, $b[k]=a[k]$. According to \cite{TeiShaSan:15}, we can construct the attack signal $\{a[k]\}_{k=0}^{\infty}$ by
\begin{equation}
    \begin{split}
        z[k+1]&=\left(A-\frac{BCA}{CB}\right)z[k],\\
        a[k]&=-\frac{CA}{CB}z[k],
    \end{split}\label{eq:pr:zda}
\end{equation}
where $z[k]\in\mathbb{R}^n$, $z[0]\in\ker(C)$ and $z[0]\neq 0$. Note that the nonminimum phase property of \eqref{eq:pr:dsys} implies that the system matrix $A-\frac{BCA}{CB}$ is unstable. The core idea of zero dynamics attacks is that this attack signal $a[k]$ will make the system states diverge but remain in the undetectable region. Regarding this type of attacks, the following result is fundamental \cite{TeiShaSan:15}.
\begin{lem}\label{lem:zda}
Consider the system in \eqref{eq:pr:dsys}. For any $\epsilon>0$, there exist attack signals such that they are $\epsilon$-stealthy and $\left\|x_{u+a}[k]-x_u[k]\right\|_2$ diverges as $k\rightarrow\infty$.
\end{lem}
